Limits of Random Oracles in Secure Computation

The seminal result of Impagliazzo and Rudich (STOC 1989) gave a black-box separation between one-way functions and public-key encryption: informally, a public-key encryption scheme cannot be constructed using one-way functions as the sole source of computational hardness. In addition, this implied a black-box separation between one-way functions and protocols for certain Secure Function Evaluation (SFE) functionalities (in particular, Oblivious Transfer). Surprisingly, however, {\em since then there has been no further progress in separating one-way functions and SFE functionalities} (though several other black-box separation results were shown). In this work, we present the complete picture for deterministic 2-party SFE functionalities. We show that one-way functions are black-box separated from {\em all such SFE functionalities}, except the ones which have unconditionally secure protocols (and hence do not rely on any computational hardness), when secure computation against semi-honest adversaries is considered. In the case of security against active adversaries, a black-box one-way function is indeed useful for SFE, but we show that it is useful only as much as access to an ideal commitment functionality is useful. Technically, our main result establishes the limitations of random oracles for secure computation.

==> detailed_frontiers_prelims.tex <==
\subsection{Additional Notations} 

Here we introduce some notation used in our proofs.
We say that $\alpha=\beta\pm\gamma$ to mean that $\abs{\alpha-\beta}\leq\abs{\gamma}$.


\subsubsection{Oracles and Query-Answer Sets}
An oracle $\cO$ is specified by a function (from queries to answers) chosen
according to a specified distribution. This choice is made before answering
any query, however for the sake of analysis of the protocol we can choose the randomness of the oracle \emph{along the way} as the parties interact (this is also known as the {\em lazy evaluation} of the oracle).
In this paper, we shall use $\cO$ which are random oracles, i.e. every query is independently mapped to an image chosen uniformly at random.

\paragraph{Security Parameter of $\cO$.} 
We shall associate a security parameter $\spar$ with the queries to  the oracle, and will invariably require that the length of the queries and
their answers is polynomial in $\spar$ (\eg $\cO$ for the security parameter $\spar$ could be a random function from $\bits^\spar$ to $\bits^\spar$). For simplicity, any protocol using the
oracle would make all queries with the same security parameter as the
protocol's own security parameter.

%
%
%
%
%
%
%
%
%
%
%
%
%
%


\paragraph{Query and Query-Answer Operators.} For any view $V$ of some
oracle algorithm interacting with $\cO$, 
we denote the set of oracle queries made by the algorithm
according to the view $V$ by $\Q(V)$.




